Contracting a Single Element in a Transversal Matroid

It is well known that the class of transversal matroids is not closed under contraction or duality. In particular, after contracting a set of elements from a transversal matroid, the resulting matroid may or may not be transversal, and the computational complexity of determining whether it is transversal is not well understood. As a step toward resolving this, we provide a polynomial-time algorithm for determining whether a single-element contraction of a transversal matroid is transversal. In the case that the single-element contraction is transversal, the algorithm also provides a transversal representation. We then discuss possible applications of our techniques toward finding a polynomial-time algorithm to determine if the dual of a transversal matroid is transversal.

==> StrictGammoids.tex <==
\section{Co-Transversal Matroids and Strict Gammoids}

\subsection{Co-Transversal Matroids}

We begin this section by calculating the dual of \eqref{betaeq}. That is, we wish to obtain a function which will be non-zero on all sets of a matroid if and only if that matroid is co-transversal.

At first, we have
\[\beta^*(Y) = r^*(M) - r^*(Y) - \sum_{Z \in \mathcal{Z}(M^*): Y \subset Z} \beta^*(Z).\]

We can use \eqref{rank dual} to get
\[\beta^*(Y) = |E(M)|-r(M) - r(\bar{Y})-|Y|+r(M) - \sum_{Z \in \mathcal{Z}(M^*): Y \subset Z} \beta^*(Z).\]

We may cancel the $r(M)$ terms and combine the cardinality terms
\[\beta^*(Y) = |\bar{Y}| - r(\bar{Y}) - \sum_{Z \in \mathcal{Z}(M^*): Y \subset Z} \beta^*(Z).\]

We wish to replace $Y$ with $\overline{Y}$ in the range of the summation. To do this note that if $Y \subset Z$ then $\overline{Z} \subset \overline{Y}$, this gives us
\[\beta^*(Y) = |\overline{Y}| - r(\overline{Y}) - \sum_{Z \in \mathcal{Z}(M^*): \overline{Z} \subset \overline{Y}} \beta^*(Z).\]

The first two terms in the sum are of course the nullity of $\overline{Y}$ which is defined as $n(\overline{Y}) = |\overline{Y}|-r(\overline{Y})$, while in the summation term it would help if we just examined $\overline{Z}$ directly. This is fortunately, quite easy, as the cyclic flats of $M$ are exactly the complements of cyclic flats of $M^*$, hence we have
$$\beta^*(Y) = n(\overline{Y}) - \sum_{Z \in \mathcal{Z}(M): Z \subset \overline{Y}} \beta^*(\overline{Z}).$$

We now relable $\overline{Y}$ to be $X$ and then we have
\[\beta^*(\overline{X}) = n(X) - \sum_{Z \in \mathcal{Z}(M): Z \subset X} \beta^*(\overline{Z}).\]

Now we define a new function $\gamma(X)$ which is simply $\beta^*(\overline{X})$, we can then replace both of our $\beta^*$ terms as follows
\begin{equation}
\label{og gamma}
\gamma(X) = n(X) - \sum_{Z \in \mathcal{Z}(M): Z \subset X} \gamma(Z)
\end{equation}
and so we obtain our $\gamma$ function. Since the $\gamma$ function checks the same sets as the $\beta^*$ function we obtain the following Corollary.

\begin{corollary}
\label{gamma}
	A matroid, $M$, is co-transversal if and only if $\gamma(X)\geq 0$ for all $X \subseteq E(M)$.
\end{corollary}

We now have a way to test if a matroid is co-transversal. We will next describe the class of strict gammoids and prove that not only are they co-transversal but that they are exactly the class of co-transversal matroids. That is, we will reprove the following theorem from \cite{INGLETON197351}

Everything we are proving in this subsection is already known but we require certain formulations of these results which have only been proved in the dual case for transversal matroids and so we provide the direct proof in the strict gammoid case for completeness.

\subsection{Strict Gammoids}

For this section, and future sections, we refer to the ground set of a matroid as $E$ and an element of the ground set as $e$. This is standard for matroids but we mention it because the elements of our matroid will be vertices of a graph rather than edges, which are often also labelled as $e$. Our edges will be directed and so we will refer to them as arcs in order to distinguish them from elements of the matroid.

Let $D$ be a directed graph and let $S$ be a set of ``sink" vertices for $D$. We do not require that there are no outgoing arcs from vertices of $S$ as the existence of such arcs will not affect the matroid we will construct. We say a set of vertices, $I \subseteq V(D)$ has a {\em linking} into $S$ if there exists a set of $|I|$ disjoint directed paths, each beginning at a vertex in $I$ and ending at a vertex in $S$. Note that a path may consist of a single vertex if that vertex is in both $I$ and $S$.

If $D$ is a directed graph and $E$ and $S$ subsets of the vertex set of $D$ then the set system consisting of the subsets of $E$ with linkings into $S$ is a matroid, $M$, called a {\em gammoid}, and denoted $M(D,E,S)$ \cite{mason}. In the case where $E=V(D)$ we call $M$ a {\em strict gammoid}.

Let $e$ be a vertex of a directed graph $D$. We call the set of vertices, $v$, such that $(e,v) \in A(D)$ the {\em forward neighbourhood} of $e$, denoted $N^+_D(e)$. We call the set $N^+_D(e)+e$ the {\em closed forward neighbourhood} of $e$ and denote it $N^+_D[e]$.

We construct a multiset, $\mathcal{N}$. For each vertex, $e \in V(D)-S$, we add $N^+_D[e]$ to $\mathcal{N}$ and label it $N_e$. In this way we have a set system where instead of indexing over $[n]$ we index over $V(D)-S$. Thus the set $N_{e'} \in \mathcal{N}$ is the closed forward neighbourhood, $N^+_D[e']$. This means that any bijection from elements of $V(D)$ to sets in $\mathcal{N}$ will be a map from $V(D)-S$ rather than a map from $V(D)$ to $[n]$. We can construct such a bijection, $\phi_0$, from $V(D)-S$ to $\mathcal{N}$ by letting $\phi_0(e)=e$. Therefore we show that $V(D)-S$ is a transversal of $\mathcal{N}$.

% May want to use $(N_e)_{e \in V(D)-S}$

We first have the following Proposition from \cite{combigeo}:

\begin{proposition}
\label{basis proposition}
    A set $B$ is a basis of $M(D,V(D),S)$ if and only if $\overline{B}$ is a transversal of $(V(D), \mathcal{N})$.
\end{proposition}


We see that if we have a strict gammoid we can construct the dual of it as a transversal matroid by taking the set system $(V(D),\mathcal{N})$ by Proposition~\ref{basis proposition}. Therefore we have shown one direction of Theorem~\ref{cotrans}.

To show the other direction we first have a few preliminary results.

\begin{proposition}
\label{rank in gammoid}
    Let $M=M(D,V(D),S)$ be a strict gammoid and let $Y$ be a subset of vertices of $V(D)$. Let $X \subseteq Y$ be the set of vertices such that $x \in X$ if and only if $x \notin S$ and $N^+_D[x] \subseteq Y$. Then $r_M(Y) \leq |Y-X|$.
\end{proposition}
\begin{proof}
    By the definition of a strict gammoid we have that $r_M(Y)$ is equal to the maximum number of disjoint directed paths, each beginning at a vertex in $Y$ and ending at a vertex in $S$. Let $\mathcal{P}$ be a maximum set of such paths.

    Let $P$ be one of the paths of $\mathcal{P}$. Let $y$ be the last vertex of $P$ in $Y$. We show by contradiction that $y \notin X$. Assume for contradiction that $y \in X$. Since $X \cap S=\emptyset$ we have that $y \notin S$ and so there must be at least one vertex, $z$, that is on $P$ after $y$. Therefore there is some vertex, $z'$, that is directly after $y$ on $P$ and since $y$ is the last vertex of $P$ in $Y$ we have that $z' \notin Y$. Therefore the arc $(y,z')$ is in $A(D)$. Therefore $N^+_D[y] \not \subseteq Y$ and so $y \notin X$, a contradiction. Therefore $P$ has at least one vertex, $y$ in $Y-X$. Therefore every path of $\mathcal{P}$ contains at least one vertex of $Y-X$ and since all such paths are distinct this means that $|\mathcal{P}| \leq |Y-X|$ as required.
\end{proof}

We now take a co-transversal matroid and construct a strict gammoid from it in the following way. Let $M$ be a co-transversal matroid. This of course means that all $\gamma$ values of subsets of $M$ are nonzero by Corollary~\ref{gamma}. We will construct our strict gammoid from our set of cyclic flats with non-zero $\gamma$ values. For each such cyclic flat, $X$, we will construct $\gamma(X)$ closed forward neighbourhoods equal to that cyclic flat. To do this we need an element for each set in our set system that will serve as the vertex whose closed forward neighbourhood will equal the set. That is, we need a transversal for $\mathcal{N}$ and a matching, $\phi_0$, of that transversal.

\begin{proposition}
\label{phi0 matching}
    Let $M$ be a co-transversal matroid and let $\mathcal{A}$ be the set system of cyclic flats of $M$ with nonzero $\gamma$ values, each with multiplicity equal to its $\gamma$ value. There exists a transversal with matching, $\phi_0$, of $\mathcal{A}$ from the elements of $E(M)$.
\end{proposition}
\begin{proof}
    We will show that for all subcollections, $\mathcal{A}' \subseteq \mathcal{A}$ we have that
    \[
    |\cup \mathcal{A}'| \geq |\mathcal{A}'|.
    \]
    and the result will follow from Theorem~\ref{hall}.

    That is, for every subcollection, $\mathcal{A}'$, the cardinality of the union of sets in that collection is at least the number of sets in that collection.

    Let $\mathcal{A}'$ be a subcollection and let $\mathcal{A}'_0$ be the union of $\mathcal{A}'$ with all sets, $A$, in $\mathcal{A}$ for which $A \subseteq \cup \mathcal{A}'$. Since every set we add gives us no new elements in $E(M)$ doing this will give us $|\mathcal{A}'|\leq |\mathcal{A}'_0|$ but $|\cup \mathcal{A}'|=|\cup \mathcal{A}'_0|$. Therefore it suffices to show that
    \[
    |\cup \mathcal{A}'_0| \geq |\mathcal{A}'_0|.
    \]

    Since the mulitiplicity in $\mathcal{A}$ of any set is equal to its $\gamma$ value and for any set in $\mathcal{A}'_0$ all copies of that set are in $\mathcal{A}'_0$ by construction we have that
    \[
    |\mathcal{A}'_0|=\sum_{A \in \mathcal{A}'_0} \gamma(A)
    \]
    but because the sets $A \in \mathcal{A}'_0$ are exactly the sets contained in $\cup \mathcal{A}'$ this is
    \[
    |\mathcal{A}'_0|=\sum_{A \in \mathcal{A}: A \subseteq \cup \mathcal{A}'} \gamma(A)
    \]
    and of course since all cyclic flats in $M$ either have a $\gamma$ value of 0 or are in $\mathcal{A}$ this means we are actually summing over all cyclic flats in $M$ contained in $\cup \mathcal{A}'$. That is
    \[
    |\mathcal{A}'_0|=\sum_{Z \in \mathcal{Z}(M): Z \subseteq \cup \mathcal{A}'} \gamma(Z).
    \]

    There are two cases, either $\cup \mathcal{A}'$ is a cyclic flat in $M$ with nonzero $\gamma$ value. Or $\cup \mathcal{A}'$ is not a cyclic flat in $M$ with nonzero $\gamma$ value. In the first case $\gamma(\cup \mathcal{A}')$ appears in the sum and so may remove it from the sum, changing the range from $Z \subseteq \cup \mathcal{A}'$ to $Z \subset \cup \mathcal{A}'$
    \[
    |\mathcal{A}'_0|=\gamma(\cup \mathcal{A}') + \sum_{Z \in \mathcal{Z}(M): Z \subset \cup \mathcal{A}'} \gamma(Z).
    \]
    Which, by \eqref{og gamma} implies that
    \[
    |\mathcal{A}'_0|=n(\cup \mathcal{A}')
    \]
    and since $n(\cup \mathcal{A}') \leq |\cup \mathcal{A}'|$ we obtain the result in this case. In the second case $\gamma(\cup \mathcal{A}')$ is not in the sum and so we have
    \[
    |\mathcal{A}'_0|=\sum_{Z \in \mathcal{Z}(M): Z \subset \cup \mathcal{A}'} \gamma(Z).
    \]
    Which, by \eqref{og gamma} implies that
    \[
    |\mathcal{A}'_0|=n(\cup \mathcal{A}') - \gamma(\cup \mathcal{A}')
    \]
    and since $\gamma(\cup \mathcal{A}') \geq 0$ and $n(\cup \mathcal{A}') \leq |\cup \mathcal{A}'|$ we obtain the result in this case as well.
\end{proof}

Let $M$ be a co-transversal matroid. Let $\phi_0$ be the matching obtained by Proposition~\ref{phi0 matching}. We now construct our strict gammoid from $\phi_0$, such that the resultant strict gammoid will represent $M$. We construct a directed graph $D$ with vertex set equal to $E(M)$. Then, for each vertex, $e$ in the domain of $\phi_0$, we direct an arc from $e$ to each vertex in $\phi_0(e)-e$. This means that $N^+_D[e]=\phi_0(e)$. Recall that $\phi_0(e)$ is a set in $\mathcal{A}$ and therefore a cyclic flat of $M$ with nonzero $\gamma$ value. Hence our closed forward neighbourhoods will be exactly the cyclic flats of $M$ with positive $\gamma$ values. We now let $S$ be the set of all vertices not in the domain of $\phi_0$. That is, those vertices not used in the matching. We now prove that $M=M(D,V(D),S)$.

\begin{lemma}
\label{gammoid=cotrans}
    $M=M(D,V(D),S)$.
\end{lemma}

\begin{proof}
    We must prove two results. First that every dependent set in $M$ is dependent in $M(D,V(D),S)$ and second that every independent set in $M$ is independent in $M(D,V(D),S)$. For the first result it suffices to show that every circuit of $M$ is dependent in $M(D,V(D),S)$.

    To see this let $C$ be an arbitrary circuit of $M$ and let $cl_M(C)$ be the closure of $C$ in $M$. Note that $cl_M(C)$ is a cyclic flat of $M$ and therefore $cl_M(C) \in \{Z \in \mathcal{Z}(M): Z \subseteq cl_M(C)\}$. Therefore we may rearrange \eqref{og gamma} to obtain
    \[
    n_M(cl_M(C)) = \sum_{Z \in \mathcal{Z}(M): Z \subseteq cl_M(C)} \gamma(Z)
    \]
    where we use $\subseteq$ instead of $\subset$ since we are combining the summation term with $\gamma(cl_M(C))$.

    However, this sum is also equal to the number of sets in $\mathcal{A}$ that are contained in $cl_M(C)$ counted with multiplicity. Each of these sets has a vertex of $V(D)-S$ matched to it by $\phi_0$ and each of those vertices has a closed forward neighbourhood equal to the set it is matched with in $M(D,V(D),S)$. So there are $n_M(cl_M(C))$ vertices among the vertices representing $cl_M(C)$ whose closed forward neighbourhoods are contained in $cl_M(C)$, none of which are in $S$. Therefore the rank of $cl_M(C)$ in $M(D,V(D),S)$ is at most $|cl_M(C)|-n_M(cl_M(C))$ by Proposition~\ref{rank in gammoid}. But of course $|cl_M(C)|-n_M(cl_M(C))=r_M(cl_M(C))$, so the rank of $cl_M(C)$ in $M(D,V(D),S)$ is at most the rank in $M$ of $cl_M(C)$. Therefore the rank of $C$ in $M(D,V(D),S)$ must be at most the rank of $C$ in $M$ and so $C$ is dependent in $M(D,V(D),S)$ as required.

    We now show that any independent set in $M$ is independent in $M(D,V(D),S)$. It will suffice to show this for bases of $M$. Let $B$ be a basis of $M$.

    From Proposition~\ref{basis proposition} it suffices to show that $\overline{B}$ is a transversal of $\mathcal{A}$. By Theorem~\ref{hall} it suffices to show that
    \[
    |(\cup \mathcal{A}')-B)| \geq |\mathcal{A}'|
    \]
    where $\mathcal{A}'$ is any subcollection of $\mathcal{A}$. As in the proof of Proposition~\ref{phi0 matching} we may assume that every set of $\mathcal{A}$ contained in $\cup \mathcal{A}'$ is in $\mathcal{A}'$. This means that
    \[
    |\mathcal{A}'|=\sum_{Z \in \mathcal{Z}(M):Z \subseteq \cup \mathcal{A}'} \gamma(Z).
    \]
    
    But as in the proof of Proposition~\ref{phi0 matching} we have that 
    \[
    \sum_{Z \in \mathcal{Z}(M):Z \subseteq \cup \mathcal{A}'} \gamma(Z) \leq n_M(\cup \mathcal{A}').
    \]

    Then since $|(\cup \mathcal{A}') \cap B|$ is independent in $M$ we have that $|(\cup \mathcal{A}') \cap B| \leq r_M(\cup \mathcal{A}')$ and so $|(\cup \mathcal{A}')-B)| \geq n_M(\cup \mathcal{A}')$ and therefore we obtain the result.
\end{proof}

Lemma~\ref{gammoid=cotrans} gives us a way to construct a strict gammoid that is isomorphic to any given co-transversal matroid. Therefore we prove the other direction of Theorem~\ref{cotrans} and obtain a full proof of Theorem~\ref{cotrans}.

Note that we could also use this method with any collection of cyclic flats with nonzero $\gamma$ values provided they had a matching. If $M'$ were a matroid with a collection of cyclic flats with nonzero $\gamma$ values then we could try to obtain a matching for the cyclic flats and if we found one we could try to construct a strict gammoid as described. If $M'$ were a cotransversal matroid then the strict gammoid we constructed would equal $M'$ provided we were using all the cyclic flats of $M'$ with nonzero $\gamma$ values, however, if $M'$ was not a cotransversal matroid the strict gammoid we constructed would not be equal to $M'$ although this might not be immediately apparent. We explore this procedure later and in our case we will provide a method to determine if the original matroid and the strict gammoid constructed from it are equal or not.

We end this section with a few brief corollaries.

\begin{corollary}
\label{construct gammoid}
    Let $M$ be any matroid and let $\mathcal{F}$ be the collection of cyclic flats of $M$ with positive $\gamma$ values. If $\mathcal{F}$ does not have a transversal from the elements of $E(M)$ then $M$ is not a strict gammoid. If $\mathcal{F}$ does have a transversal from the elements of $E(M)$ then let $M'=M(D,V(D),S)$ where $D$ and $S$ are constructed as in Lemma~\ref{gammoid=cotrans}. Then if $M$ is a strict gammoid $M=M'$.
\end{corollary}
\begin{proof}
    The transversal result comes from Proposition~\ref{phi0 matching}. The rest follows from Lemma~\ref{gammoid=cotrans} and the discussion above.
\end{proof}

\begin{corollary}
\label{bound corollary}
    Let $M$ be a strict gammoid. Then
    \[
    \sum_{Z \in \mathcal{Z}(M): Z \subset E(M)} \gamma(Z) \leq n(E(M)).
    \]
\end{corollary}
\begin{proof}
    By Theorem~\ref{cotrans} we have that $M$ is co-transversal and therefore by Corollary~\ref{gamma} we have that $\gamma(E(M)) \geq 0$, substituting in \eqref{og gamma} and rearranging gives the result.
\end{proof}

\begin{corollary}
\label{poly time}
    Let $M$ be a co-transversal matroid with $k=|E(M)|$ and let $\mathcal{A}$ be its collection of cyclic flats with nonzero $\gamma$ values. Let $X$ be a set of $E(M)$. Then, given only the collection $\mathcal{A}$ along with each of their $\gamma$ values it is possible to determine whether or not $X$ is independent in polynomial time with respect to $k$.
\end{corollary}
%may not need this
\begin{proof}
    We use Lemma~\ref{gammoid=cotrans} to construct a strict gammoid representation of $M$. This can be done using only the sets in $\mathcal{A}$ and their $\gamma$ values. It can be done in polynomial time since for each set, $A$, in $\mathcal{A}$ we are adding at most $k \gamma(A)$ edges and we never have to remove edges. We also have from Corollary~\ref{bound corollary} that both $\gamma(A)$ and $|\mathcal{A}|$ are bounded by $k$. We can then use standard maximum flow algorithms \cite{bondyandmurty} to determine in polynomial time if $X$ has a linking to $S$.
\end{proof}

This justifies the techniques we will use which deal mostly with the collection $\mathcal{A}$ and $\gamma$ values of its members. However, we must also consider the case when we are given a strict gammoid in the form of a directed graph. How do we obtain $\mathcal{A}$ in polynomial time? We have shown a method to obtain a strict gammoid from the collection $\mathcal{A}$ complete with its $\gamma$ values, however we have not shown that the reverse is possible. We will demonstrate how this is done in the next subsection. The techniques used there are related to the graphical representations of strict gammoids and gammoids and we shall not use such techniques for our proofs in the later sections but we provide them for completeness.

\subsection{Directed Graph Properties}

Let $D$ be a directed graph with sink set $S \subseteq V(D)$. 

\begin{lemma}
\label{first closure lemma}
    Let $M=M(D,V(D),S)$ be a strict gammoid. Let $I$ be an independent set in $M$ and let $e$ be a vertex in $cl(I)-I$. Let $\mathcal{P}$ be a set of paths linking $I$ into $S$ such that $e$ is on no path of $P$. Then $N^+_D[e] \subseteq cl(I)$.
\end{lemma}
\begin{proof}
    Let $f$ be a vertex in $N^+_D[e]$. Assume for contradiction that $f \notin cl(I)$. This means that $I+f$ is independent in $M$. Let $\mathcal{P}_f$ be a set of paths linking $I+f$ into $S$ and let $P_f$ be the path of $\mathcal{P}_f$ that begins at $f$. If no path of $\mathcal{P}_f$ intersects $e$ then we may extend $P_f$ backward by one vertex to $e$ since there is an arc from $e$ to $f$ in $D$. We would then have a set of paths linking $I+e$ into $S$, contradicting the fact that $e \in cl(I)$. Therefore we assume that there is some path, $P_e$, of $\mathcal{P}_f$ that intersects $e$. Let the first vertex of $P_e$ be $v_0$.

    We now construct a linking, $\mathcal{P}_e$, of $I+e$. To do this first add all paths from $\mathcal{P}_f$ to $\mathcal{P}_e$ except for the part of $P_e$ before $e$. That is, the part of $P_e$ from $v_0$ to $e$. This gives us a set of paths linking $I+e+f-v_0$ into $S$. We will be done when we can add a path from $v_0$ into this set of paths while maintaining paths from all other vertices, except perhaps $f$.

    To do this note that $v_0 \in I$ and therefore there is some path, $P_0 \in \mathcal{P}$ which links $v_0$ to $S$ and does not intersect $e$. This is the only property we need and all the following arguments can be repeated for any vertex in $I$. We add $P_0$ to $\mathcal{P}_e$ arc by arc until we either reach $S$, in which case we are done, or until we intersect some other path already in $\mathcal{P}_e$. As we add these arcs and vertices we colour them red.

    Assume that the path we are adding intersects with a path already in $\mathcal{P}_e$. Note that the path we are adding, which is red, cannot intersect any other red path since all red paths are in $\mathcal{P}$ and so do not intersect each other. Let the non-red path we have intersected with be $P_0'$ and let the first vertex of $P_0'$ be $v_1$. We have three possibilities for $v_1$. First we could have $v_1=f$ in which case we let $P_0$ follow $P_0'$ after they intersect and remove the earlier part of $P_0'$ from $\mathcal{P}_e$. We will therefore obtain a linking of all the vertices in $I+e+f$ except for $f$ and therefore obtain a linking of $I+e$ as required. If this happens we are done so in all other cases we can assume we still have a path from $f$ to $S$ in our set of paths. The second case is that $v_1=e$. In this case similarly we let $P_0$ follow $P_0'$ after they intersect and remove the part of $P_0'$ before the intersection from $\mathcal{P}_e$. We now have a linking of $I+f$ into $S$, however, note that $P_0$ does not intersect $e$ by construction so this is a set of paths that does not intersect $e$. We therefore extend the path from $f$ back by one vertex to $e$ and obtain our desired linking.

    The final case is that $v_1$ is not equal to either $f$ or $e$. In which case we have that $v_1 \in I$ and therefore there is a path, $P_1 \in \mathcal{P}$, that links $v_1$ to $S$ and does not intersect $e$. Similar to before we let $P_0$ follow $P_0'$ after they intersect, making sure not to colour the rest of this new path red, and we delete the earlier part of $P_0'$ from $\mathcal{P}_e$. We now begin our process again following $P_1$ from $v_1$. Note that our process never crosses a red path and so since there are only a finite number of vertices in $D$ we must finish this process. Therefore we obtain a set of paths, $\mathcal{P}_e$ that links $I+e$ into $S$. Therefore we obtain the result by contradiction.
\end{proof}

\begin{lemma}
\label{magic edge}
    Let $M=M(D,V(D),S)$ be a strict gammoid. Let $I$ be an independent set in $M$ such that for every set of paths, $\mathcal{P}$, linking $I$ into $S$ the arc $(e,f)$ appears on some path in $\mathcal{P}$. Let $\mathcal{P}$ be such a linking and let $P_e$ be the path that $(e,f)$ appears on in $\mathcal{P}$.
    
    Let $v_0$ be the first vertex of $P_e$. Then, $I'=I-v_0+e$ is independent and for every set of paths linking $I'$ into $S$ we have that $(e,f)$ appears on one of the paths.
\end{lemma}
\begin{proof}
    Note that we can shorten $P_e$ to start at $e$ and therefore obtain a linking of $I'$, hence $I'$ is clearly independent.

    Assume for contradiction that $\mathcal{P}'$ is some set of paths linking $I'$ into $S$ without using $(e,f)$. We now construct a set of paths, $\mathcal{P}''$, linking $I$ into $S$ without using $(e,f)$. To do this we first add all paths of $\mathcal{P}'$ to $\mathcal{P}''$. We now need to find a path from $v_0$ to $S$ while maintaining paths from all other vertices except perhaps $e$.

    To do this note that $v_0 \in I$ and therefore there is some path, $P_0 \in \mathcal{P}$ from $v_0$ to $S$. This is the only property we need and all the following arguments can be repeated for any vertex in $I$. We add $P_0$ to $\mathcal{P}''$ arc by arc until we either reach $S$, in which case we are done, or until we intersect some other path already in $\mathcal{P}''$. As we add these arcs and vertices we colour them red.

    Assume that the path we are adding intersects with a path already in $\mathcal{P}''$. Note that the path we are adding, which is red, cannot intersect any other red paths since all red paths are in $\mathcal{P}$ and so do not intersect each other. Let the non-red path we have intersected with be $P_0'$ and let the first vertex of $P_0'$ be $v_1$. We have two possibilities for $v_1$. First we could have $v_1=e$ in which case we let $P_0$ follow $P_0'$ after they intersect and remove the earlier part of $P_0'$ from $\mathcal{P}''$. We will then have obtained a linking of $I'+v_0-e$ which is a linking of $I$. Note that this process will prevent our path from using $(e,f)$ as in order to use this edge $P_0$ must first reach $e$ which would mean it would intersect with $P_0'$ at $e$ and by construction $P_0'$, after $e$, does not use $(e,f)$. Therefore we cannot add a path that uses $(e,f)$ to $\mathcal{P}''$.

    In the other possibility we have that $v_1 \neq e$, in which case $v_1 \in I$ and therefore there is a path, $P_1 \in \mathcal{P}$, that links $v_1$ to $S$. Similar to before we let $P_0$ follow $P_0'$ after they intersect, making sure not to colour the rest of this path red, and we delete the earlier part of $P_0'$ from $\mathcal{P}''$. We now begin our process again following $P_1$ from $v_1$. Note that our process never crosses a red path and so since there are only a finite number of vertices in $D$ we must finish this process. Therefore we obtain a set of paths, $\mathcal{P}''$ that links $I$ into $S$ without using $(e,f)$. Therefore we obtain the result by contradiction.
\end{proof}

\begin{lemma}
\label{second closure lemma}
    Let $M=M(D,V(D),S)$ be a strict gammoid. Let $I$ be an independent set in $M$ such that for every set of paths, $\mathcal{P}$, linking $I$ into $S$ the vertex $e \notin I$ appears on some path in $\mathcal{P}$. Let $\mathcal{P}$ be such a linking and let $P_e$ be the path that $e$ appears on in $\mathcal{P}$.
    
    Let $f$ be the vertex of $P_e$ before $e$ on $P_e$. Then $f \in cl(I)$.
\end{lemma}
\begin{proof}
    Assume for contradiction that $f \notin cl(I)$. Then there exists some set of paths, $\mathcal{P}_f$, linking $I+f$ into $S$. We now construct a set of paths, $\mathcal{P}_0$ that links $I$ into $S$ such that no path of $\mathcal{P}_0$ intersects $e$. To do this we first add all paths of $\mathcal{P}_f$ to $\mathcal{P}_0$. If none of these paths intersect $e$ then we are done, otherwise we assume that one of the paths, $P_0$, intersects $e$. Let the first vertex of $P_0$ be $v_0$, we now have two cases.

    In the first case $v_0=f$. In this case since we are trying to link $I$ not $I+f$ we can simply delete $P_0$ and obtain our required linking. In the second case $v_0 \neq f$ and therefore $v_0 \in I$, this means that the path from $f$ in $\mathcal{P}_0$ does not intersect $e$. Since $v_0 \in I$ there is some path, $P_0 \in \mathcal{P}$ linking $v_0$ to $S$. We add $P_0$ to $\mathcal{P}_0$ arc by arc until we either reach, $S$, in which case we are done, or until we intersect some other path already in $\mathcal{P}_0$. As we add these vertices we colour them red.

    Assume that the path we are adding intersects with a path, $P_1$, already in $\mathcal{P}_0$. We let $P_0$ follow $P_1$ after they intersect, making sure not to colour those vertices red, and we remove the part of $P_1$ before the intersection from $\mathcal{P}_0$. We then examine the first vertex of $P_1$ and repeat this process there. Once again we are guaranteed to never intersect a red path since they are all in $\mathcal{P}$, therefore this process must terminate. We are also guaranteed to never intersect $e$ since the only path in $\mathcal{P}$ that intersects $e$ intersects $f$ first and if $v_0 \neq f$ then the path from $f$ in $\mathcal{P}_f$ cannot intersect $f$ so we could follow the same procedure except we would not have to start again with new vertex $v_1$. Therefore we obtain the result.
\end{proof}

\begin{lemma}
\label{add arc}
    Let $M=M(D,V(D),S)$ be a strict gammoid. Let $e$ and $f$ be vertices of $D$ such that $(e,f) \notin A(D)$ and $e \notin S$. Then $M'=M(D+(e,f),V(D),S)=M$ if and only if $f \in cl_M(N^+_D[e])$.
\end{lemma}
\begin{proof}
    We first prove that if $f \in cl_M(N^+_D[e])$ then $M'=M$.

    Note that all sets that can be linked into $S$ in $D$ can be linked into $S$ in $D+(e,f)$ by the same paths. Therefore it suffices to show that no set is dependent in $M$ and independent in $M'$. For contradiction assume that $I$ is such a set. Note that every set of paths, $\mathcal{P}$, linking $I$ into $S$ in $D+(e,f)$ must use the arc $(e,f)$ as otherwise those paths would exist in $D$ and $I$ would be independent in $M$. Let $P_e$ be the path of $\mathcal{P}$ that uses $(e,f)$ and let $v$ be the first vertex of $P_e$. By Lemma~\ref{magic edge} we also have that $I'=I-v+e$ is independent in $M'$ and has the property that any set of paths linking $I'$ into $S$ uses $(e,f)$. Therefore $I'$ must be dependent in $M$. Therefore to obtain our contradiction it suffices to examine $I'$ instead of $I$.

    Note that since $e \in I'$ and the edge $(e,f)$ is used in every set of paths linking $I'$ into $S$ there exists a set of paths, $\mathcal{P}_e$, linking $I'$ into $S$ where the path, $P_e'$ linking $e$ to $S$, contains $(e,f)$. Note that $\mathcal{P}_e-P_e'$ is a linking of $I'-e$ that does not use the arc $(e,f)$ and therefore exists in $D$. Hence $I'-e$ is independent in $M$ but $I'$ is not. Therefore $e \in cl_M(I'-e)$. Furthermore $\mathcal{P}_e - P_e'$ is a linking of $I'-e$ that does not intersect $e$ at all. Therefore by Lemma~\ref{first closure lemma} we have that $N^+_D[e] \subseteq cl_M(I'-e)$.

    However, since the first arc of $P_e'$ is $(e,f)$ we can shorten it to start at $f$ instead of $e$ and obtain a set of paths linking $I'-e+f$ into $S$ that does not use the arc $(e,f)$ and therefore exists in $D$. Therefore $I'-e+f$ is independent in $M$ and so $f \notin cl_M(I'-e)$. However $f \in cl_M(N^+_D[e])$ and $N^+_D[e] \subseteq cl_M(I'-e)$, and so $cl_M(N^+_D[e]) \subseteq cl_M(I'-e)$ therefore we obtain our contradiction.

    For the other direction assume that $f \notin cl_M(N^+_D[e])$. Let $\mathcal{P}$ be a set of paths that links the maximum number of vertices in $N^+_D[e]$ into $S$. Let the set of vertices at the beginning of paths in $\mathcal{P}$ be $I$. Note that $r_M(N^+_D[e])=|I|$. Observe that we may assume for any such linking of any such $I$ that $e$ does not appear on any path of $\mathcal{P}$ as if $e \in P$ for some $P \in \mathcal{P}$ then let $e'$ be the vertex after $e$ in $P$. Such a vertex exists since $e \notin S$ so $P$ cannot end at $e$. We then obtain a new linking for a new independent set by shortening $P$ to start at $e'$. Since $e' \in N^+_D[e]$ this new independent set is a maximum sized independent set contained in $N^+_D[e]$ as required.

    Note that $f \notin cl_M(N^+_D[e])$ and therefore if $I$ is a maximum sized independent set contained in $N^+_D[e]$ we have that $f \notin cl_M(I)$. Therefore there exists a linking, $\mathcal{P}_f$, of $I+f$ in $D$. Let $P_f$ be the path of $\mathcal{P}_f$ that begins at $f$. Note that $\mathcal{P}_f-P_f$ is a linking of a maximum sized independent set contained in $N_D^+[e]$ and so we can assume, as above, that no path of $\mathcal{P}_f-P_f$ passes through $e$. We also see that $P_f$ does not pass through $e$ as if it did we could shorten it to start at $e$ and obtain a linking of $I+e$, contradicting the fact that $I$ was a maximum sized independent set contained in $N^+_D[e]$. Therefore no path of $\mathcal{P}_f$ passes through $e$.

    This means that in $D+(e,f)$ we can extend $P_f$ backward to $e$ through the arc $(e,f)$ and obtain a linking of $I+e$. Therefore $r_{M'}(N^+_D[e])>r_M(N^+_D[e])$ and therefore $M' \neq M$ as required.
\end{proof}

Lemma~\ref{add arc} gives us a way to add arcs to our strict gammoids without changing the strict gammoid. If $D_M$ is a directed graph representation of a strict gammoid, $M$, such that there are no arcs from vertices in $S$ and adding any arc from a vertex $e \notin S$ to $D_M$ prevents it from being a representation of $M$ then we say that $D_M$ is a {\em maximal representation}.Since we can determine closures of given sets in polynomial time for a given representation it is easy to obtain a maximal representation of a strict gammoid in polynomial time. We simply use Lemma~\ref{add arc} to determine if we can add an arc or not for each missing arc of which there are at most $\mathcal{O}(n^2)$ where $n$ is the number of vertices.

\begin{lemma}
    Let $M=M(D,V(D),S)$ be a strict gammoid. Let $D_M$ and $D_M'$ be maximal representations for $M$ obtained by adding arcs to $D$ and removing arcs from vertices in $S$. Then $D_M=D_M'$.
\end{lemma}
\begin{proof}
    Let $D'$ be a representation obtained from $D$ by adding all arcs that can possibly be added using Lemma~\ref{add arc}. Then if $N^+_D[e]$ is a closed forward neighbourhood of a vertex $e$ in $D$ we must have that $N^+_{D'}[e]=cl_M(N^+_D[e])$. Since both $D_M$ and $D_M'$ must be obtained in this way and by the "only if" condition on Lemma~\ref{add arc} we cannot add any other arcs, we have that $N^+_{D_M}[e]=N^+_{D_M'}[e]$ for all $e \notin S$ and since there are no arcs from vertices in $S$ we also have that $N^+_{D_M}[s]=N^+_{D_M'}[s]$ for all $s \in S$. Therefore $D_M=D_M'$.
\end{proof}

Observe that in a maximal representation every closed forward neighbourhood must be a flat as if there is some element in the closure of such a neighbourhood it must be in the neighbourhood.

\begin{corollary}
\label{union corollary}
    Let $M=M(D,V(D),S)$ be a strict gammoid and let $Z$ be a cyclic flat of $M$. Then $Z$ is a union of closed forward neighbourhoods of $D$.
\end{corollary}
\begin{proof}
    Since any cyclic flat is a union of closures of circuits it suffices to prove that a closure of a circuit is a union of closed forward neighbourhoods.

    Let $C$ be a circuit in $M$ and let $cl(C)$ be its closure. Let $e$ be a vertex in $cl(C)$. Let $I$ be a maximum independent set of $C$ that does not contain $e$, since $C$ is a circuit such a set exists. We have two cases.
    
    First, assume that there is some set of paths, $\mathcal{P}$, linking $I$ into $S$ such that no path of $\mathcal{P}$ intersects $e$. If $e \in S$ then we may simply add $e$ to $I$ and obtain an independent set and so $e \notin cl(I)$, a contradiction. Therefore we have that $e \notin S$ and so by Lemma~\ref{first closure lemma} we have that $N^+_D[e] \subseteq cl(I)$ and so there is a closed forward neighbourhood in $cl(C)$ that contains $e$.

    In the second case we assume that in every set of paths, $\mathcal{P}$, linking $I$ into $S$, there is a path, $P_e$, that intersects $e$. Let $f$ be the first vertex of $P_e$ and let $f'$ be the vertex of $P_e$ before $e$. By Lemma~\ref{second closure lemma} we have that $f' \in cl(I)$ and therefore $f' \in cl(C)$. Since $e \in cl(C)$ and $cl(I)=cl(C)$ we have that $cl(I+e)=cl(C)$. We also have that $I-f+e$ is independent since we can obtain a set of paths linking $I-f+e$ into $S$ from $\mathcal{P}$ by simply shortening $P_e$ to start at $e$ instead of $f$. Therefore, since $I$ is a maximum sized independent set contained in $cl(C)$ we have that $I-f+e$ is also a maximum sized independent set contained in $cl(C)$. Therefore $cl(C)=cl(I-f+e)$. Note that $f' \in cl(I-f+e)$ since $f' \in cl(C)$ and we have just found a set of paths linking $I-f+e$ into $S$ such that none of the paths intersect $f'$. Therefore by Lemma~\ref{first closure lemma} we have that $N^+_D[f'] \subseteq cl(I-f+e)$ and so there is a closed forward neighbourhood in $cl(C)$ containing $e$.

    So in both cases $e$ is contained in some closed forward neighbourhood contained in $cl(C)$. Therefore $cl(C)$ is a union of closed forward neighbourhoods as required.
\end{proof}

\begin{proposition}
\label{cyclic proposition}
    Let $e$ be a vertex of $V(D)-S$. Then $N^+_D[e]$ is cyclic in $M$.
\end{proposition}
\begin{proof}
    Let $\mathcal{B}_N$ be the collection of maximal independent sets contained in $N^+_D[e]$. It suffices to show that no element in $N^+_D[e]$ appears in every set in $\mathcal{B}_N$.

    We first show that $e$ does not appear in every set in $\mathcal{B}_N$. Let $B_0$ be some set in $\mathcal{B}_N$ and let $\mathcal{P}_0$ be a set of paths linking $B_0$ to $S$ in $D$. If $e \notin B_0$ then we are done. Otherwise there is some path, $P_e \in \mathcal{P}_0$ beginning at $e$ and ending at a vertex in $S$. Since $e \notin S$ there is some vertex, $f$, on $P_e$ such that $P_e$ uses the arc $(e,f)$. Since there is an arc $(e,f) \in A(D)$ we have that $f \in N^+_D[e]$ and since a path goes through $f$ we have that $f \notin B_0$. If we shorten $P_e$ to start at $f$ instead of $e$ we obtain a new set of paths linking $B_0-e+f$ into $S$. Therefore $B_0-e+f$ is an independent set and since it has the same size as $B_0$ is in $\mathcal{B}_N$. Therefore $e$ is not in every set of $\mathcal{B}_N$.

    Now let $f$ be some element in $N^+_D[e]$ such that $f\neq e$. We now show that $f$ is not in every set in $\mathcal{B}_N$. This time let $B_1$ be some set of $\mathcal{B}_N$. If $f \notin B_1$ then we are done so we assume that $f \in B_1$. This means that there is some set of paths $\mathcal{P}_1$, linking $B_1$ into $S$ and one of these paths, $P_f$, begins at $f$. If $e$ appears on no paths of $\mathcal{P}_1$ then let $B_1'=B_1$. Otherwise let $P_e$ be the path of $\mathcal{P}_1$ that $e$ appears on. Let the first vertex of $P_e$ be $e'$ and let the vertex after $e$ on $P_e$ be $f'$. Note that since $f'$ is not the first vertex on its path $f' \neq f$. We obtain a new set of paths, $\mathcal{P}_1'$, by shortening $P_e$ to start at $f'$ instead of $e'$. Since the arc $(e,f') \in A(D)$ we have that $f' \in N^+_D[e]$ and so as before the set, $B_1'$, linked by $\mathcal{P}_1'$ is a maximal independent set of $N^+_D[e]$ and therefore $B_1' \in \mathcal{B}_N$. We have that $B_1'=B_1-e'+f'$. If $e'=f$ then we are done, otherwise, in both cases, we now have a set $B_1' \in \mathcal{B}_N$ with a set of paths, $\mathcal{P}_1'$, linking it into $S$ such that no path of $\mathcal{P}_1'$ intersects $e$ and one path, $P_f$, which starts at $f$.

    Since $f \in N^+_D[e]$ the arc $(e,f) \in A(D)$ and so we may extend $P_f$ back one arc by adding $(e,f)$ to it and therefore making $P_f+(e,f)$ a path that links $e$ to $S$. Since no path of $\mathcal{P}_1'$ intersects $e$ adding this edge still results in a linking. Therefore $B_1'-f+e$ is another maximal independent set of $N^+_D[e]$ and so $B_1'-f+e \in \mathcal{B}_N$. Therefore $f$ is not in every set in $\mathcal{B}_N$ and therefore we obtain the result.
\end{proof}

\begin{proposition}
\label{max null prop}
    Let $X$ be a flat of $M$.  Let $X_N$ be the set of vertices of $X$ in $V(D)-S$ whose closed forward neighbourhoods are contained in $X$. Then $n(X)=|X_N|$.
\end{proposition}
\begin{proof}
    Let $B_X$ be a maximal independent set in $X$. Let $\mathcal{P}$ be a set of paths linking $B_X$ to $S$ in $D$. Let $x$ be an element of $X-X_N$ that does not appear on any path of $\mathcal{P}$. Since $B_X$ is a maximal independent set in $X$ we have that $X \in cl(B_X)$ and so $x \in cl(B_X)$, therefore by Lemma~\ref{first closure lemma} we have that $N^+_D[x] \subseteq cl(B_X)$, therefore $N^+_D[x] \subseteq cl(X)$ and so since $X$ is a flat $N^+_D[e] \subseteq X$. This contradicts the fact that $x \notin X_N$. Therefore every vertex $x$ in $X-X_N$ appears on some path of $\mathcal{P}$.

    Now let $\mathcal{P}'$ be the set of paths obtained from $\mathcal{P}$ in the following way. Let $P_0$ be a path in $\mathcal{P}$ and let $x_0$ be the last vertex of $X$ on $P_0$. That is, if $e$ is the first vertex of $P_0$ then the only vertices on $P_0$ that can be in $X$ are those between $e$ and $x_0$ inclusive, on $P_0$. Observe that $x_0$ cannot be in $X_N$ as then it would not be in $S$ and so there would be some vertex $x_1$ on $P_0$ directly after $x_0$ and so $x_1$ would be in $N^+_D[x_0]$. Therefore if $x_0$ was in $X_N$ we would have that $x_1$ would be in $X$, contradicting the fact that $x_0$ is the last vertex in $X$ on $P_0$.
    
    We shorten $P_0$ to begin at $x_0$ instead of at $e$ and then we add $P_0$ to $\mathcal{P}'$. We do this for every path in $\mathcal{P}$ and therefore we obtain the same number of paths in $\mathcal{P}'$. Since all paths in $\mathcal{P}'$ start at vertices in $X$ and there are the same number of them as in $\mathcal{P}$ we have that the set $\mathcal{P}'$ links, $B_X'$, is a maximal independent set in $X$. Therefore, by our above argument each $x_0 \in X-X_N$ must appear on a path of $\mathcal{P}'$. However, by construction each path of $\mathcal{P}'$ has exactly one vertex of $X-X_N$ on it. Therefore there are exactly $|X-X_N|$ paths in $\mathcal{P}'$ and so $r(X)=|X-X_N|$ and therefore $n(X)=|X_N|$.
\end{proof}

Let $D$ be a directed graph and let $X$ be a subset of $V(D)$. We define $N_c(X)$ to be the set of vertices, $e \in V(D)$, such that $N^+_D[e]\subseteq X$. We define $N(X)$ to be the set of vertices, $e \in V(D)$, such that $N^+_D[e]=X$. Finally if $M$ is a matroid and $X$ is a subset of the ground set of $M$ we define $Z_c(X)$ to be the number of cyclic flats of $M$ contained in $X$.

\begin{theorem}
\label{theorem 23}
    Let $D_M$ be a maximal representation of a strict gammoid, $M$. Let $X$ be a subset of $E(M)$. Then $X$ is a closed forward neighbourhood of $D_M$ if and only if $X$ is a cyclic flat of $M$ with nonzero $\gamma$ value and $|N(X)|=\gamma(X)$.
\end{theorem}
\begin{proof}
    We prove this by induction on $|N_c(X)|+|Z_c(X)|$.

    For the base case let $X$ be a set that contains no cyclic flats of $M$ and no closed forward neighbourhoods of $D_M$. This means that $X$ cannot be a cyclic flat or a closed forward neighbourhood and so we prove the base case.

    For the induction step let $X$ be either a closed forward neighbourhood or a cyclic flat with nonzero $\gamma$ value and assume the result holds for all closed forward neighbourhoods and cyclic flats with nonzero $\gamma$ value strictly contained in $X$. For the first direction let $X$ be a closed forward neighbourhood. Then by Proposition~\ref{cyclic proposition} we have that $X$ is cyclic and by Lemma~\ref{add arc} we have that $X$ is a flat since $D_M$ is a maximal representation. Therefore $X$ is a cyclic flat. All that remains to show is that $|N(X)|=\gamma(X)$. Before we do this we examine the other direction. In this case let $X$ be a cyclic flat, then by Corollary~\ref{union corollary} we have that $X$ is a union of closed forward neighbourhoods. All that remains is to show that $|N(X)|=\gamma(X)$.

    In both cases observe that for each closed forward neighbourhood, $Y=N^+_D[e]$ strictly contained in $X$ we have that $|N(Y)|=\gamma(Y)$ by induction. We also have that for each cyclic flat $Y$ strictly contained in $X$ that either $\gamma(Y)=0$ or $|N(Y)|=\gamma(Y)$ by induction. Therefore the total number of closed forward neighbourhoods strictly contained in $X$ is exactly
    \[
    \sum_{Z \in \mathcal{Z}(M): Z\subset X} \gamma(Z).
    \]
    Observe that the number we have just calculated is precisely the difference between $|N_c(X)|$ and $|N(X)|$ since $N_c(X)$ includes all such neighbourhoods and $N(X)$ does not. Therefore
    \[
    |N(X)|=|N_c(X)|-\sum_{Z \in \mathcal{Z}(M): Z\subset X} \gamma(Z).
    \]
    But by Proposition~\ref{max null prop} since in both cases $X$ is a flat we have that $|N_c(X)|=n(X)$ and so this is actually
    \[
    |N(X)|=n(X)-\sum_{Z \in \mathcal{Z}(M): Z\subset X} \gamma(Z)=\gamma(X)
    \]
    as required.
\end{proof}

Therefore we can take any strict gammoid presented to us as a directed graph and obtain the maximal representation from which we can read off $\mathcal{A}$ and the $\gamma$ values of each set in $\mathcal{A}$, all in polynomial time.
